Finite element discretization of the steady, generalized Navier-Stokes equations with inhomogeneous Dirichlet boundary conditions

We propose a finite element discretization for the steady, generalized Navier-Stokes equations for fluids with shear-dependent viscosity, completed with inhomogeneous Dirichlet boundary conditions and an inhomogeneous divergence constraint. We establish (weak) convergence of discrete solutions as well as a priori error estimates for the velocity vector field and the scalar kinematic pressure. Numerical experiments complement the theoretical findings.

==> header-packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
% For debugging: find odd character
%\DeclareUnicodeCharacter{0301}{*************************************}

\usepackage{enumerate, enumitem}
\usepackage{lmodern, microtype}
\usepackage{graphicx}
\usepackage{verbatim}

\usepackage{amsmath, amsthm, amssymb, bm, esint, mathtools, xfrac}
\usepackage[bb=dsserif]{mathalpha}

\usepackage[usenames,dvipsnames]{color}
\PassOptionsToPackage{usenames, dvipsnames}{color}
\usepackage{tikz}
\usetikzlibrary{shapes,positioning}

\usepackage[english, ngerman]{babel}

\usepackage[backend=biber,style=alphabetic]{biblatex}
\usepackage{csquotes}

\usepackage[%
pdfpagelabels=true,
unicode=true,
colorlinks=false,
pdfborder={0 0 0}
]{hyperref}

%\usepackage{scrlayer-scrpage}
%\usepackage{fancyhdr}
%\pagestyle{fancy}
%\fancyhf{}
%\chead{\footnotesize{\rightmark}}
%\renewcommand{\headrulewidth}{0.5pt}
%\cfoot{\thepage}
